Computational Discovery of Chiasmus in Ancient Religious Text

Chiasmus, a debated literary device in Biblical texts, has captivated mystics while sparking ongoing scholarly discussion. In this paper, we introduce the first computational approach to systematically detect chiasmus within Biblical passages. Our method leverages neural embeddings to capture lexical and semantic patterns associated with chiasmus, applied at multiple levels of textual granularity (half-verses, verses). We also involve expert annotators to review a subset of the detected patterns. Despite its computational efficiency, our method achieves robust results, with high inter-annotator agreement and system precision@k of 0.80 at the verse level and 0.60 at the half-verse level. We further provide a qualitative analysis of the distribution of detected chiasmi, along with selected examples that highlight the effectiveness of our approach.

==> New_Figures/algo.tex <==
% \documentclass{article}
% \usepackage{algorithm}
% \usepackage{algpseudocode}

% \begin{document}

% \usepackage{algpseudocode}

% \begin{algorithm}[t]
% \footnotesize
% \begin{algorithmic}[1]
% \REQUIRE Cosine similarity matrix $cos\_sim$, starting index $i$, submatrix size $n$
% \STATE Extract the submatrix $chiasm$ from $cos\_sim[i:i+n, i:i+n]$
% \STATE Reverse the diagonal of $chiasm$
% \STATE Compute the trace of the reversed diagonal as $score$
% \IF {$n$ is odd}
%     \STATE Subtract the middle element of the diagonal from $score$
% \ENDIF
% \IF {$n$ is even}
%     \STATE Set $div = n$
% \ELSE
%     \STATE Set $div = n-1$
% \ENDIF
% \STATE Calculate the penalty $neg\_score$ as the sum of non-diagonal elements in the first and last rows of $chiasm$
% \STATE Normalize the score by dividing $score$ and $neg\_score$ by $div$
% \STATE Adjust the final score by subtracting the normalized $neg\_score$ from the normalized $score$
% \RETURN Final normalized score
% \end{algorithmic}
% \caption{Calculate Chiasm Score}
% \label{algo:chiasm}
% \end{algorithm}


\begin{algorithm}[t]
\footnotesize
\caption{Chiasm Detection}
\begin{algorithmic}[1]
\REQUIRE Cosine matrix $M$, chiasm length $n$, book breaks $B$

% \textbf{Output:} List of outlier chiasms
\STATE Initialize $S \gets \{\}$ \COMMENT{Chiasm scores}
\FOR{$i = 1$ to $m - n$} 
    \IF{$i+n$ crosses book break $B$}
        \STATE $S[i] \gets 0$
    \ELSE
        \STATE \small Compute $pair(i,n)$ and $non\_pair(i,n)$
        \STATE  $S[i] \gets avg(pair(i,n)) - avg(non_pair(i,n))$
    \ENDIF
\ENDFOR
\STATE Compute Z-scores for all $S[i]$ and identify outliers
\end{algorithmic}
\end{algorithm}

% \end{document}

